PACIT: Unlocking the Power of Examples for Better In-Context Instruction Tuning

Instruction tuning enhances the instruction following ability of large language models by finetuning with supervised instruction data. Previous work proposes in-context instruction tuning (ICIT) where specific positive or negative examples are incorporated into the prompt for better performance. In this work, we propose PACIT, a simple and effective in-context instruction tuning method, inspired by the pedagogical concept of desirable difficulty. The PACIT method unlocks the power of examples by encouraging the model to actively learn to grasp the distinctions between the positive and negative examples instead of merely reading. The model is expected to first verify the correctness of the provided example according to the task description, which is then set as the condition for generating a better response to the task instance. Our extensive experiments prove the effectiveness of PACIT, outperforming ICIT baseline on both in-domain and out-domain tasks up to 9.16 and 3.14 average ROUGE-L scores, respectively. Moreover, PACIT can notably enhance the performance of instruction tuning even when all positive and negative examples are generated with a self-instruct method.

==> stage_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\renewcommand{\arraystretch}{1.5}
\captionof{table}{The performance (ROUGE-L) under zero-shot and few-shot settings for three training methods on hold-out and hold-out datasets.}
\label{EoT performance}
\resizebox{\linewidth}{!}
{
\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{Model size} & \multirow{2}{*}{Stage} & \multicolumn{1}{l}{\multirow{2}{*}{Zero-Shot}} & \multirow{2}{*}{Few-Shot} & \multirow{2}{*}{Avg ROUGE-L} \\
                            &                        & \multicolumn{1}{l}{}                           &                           &                             \\ \hline
\multirow{2}{*}{770M}       & Separated              & \textbf{40.688}                                & 29.113                    & 34.900                      \\
                            & Combined               & 33.585                                         & \textbf{46.665}           & \textbf{40.125}             \\ \hline
\multirow{2}{*}{3B}         & Separated              & 42.821                                         & 43.4                      & 43.110                      \\
                            & Combined               & \textbf{43.09}                                 & \textbf{52.111}           & \textbf{95.201}             \\ \hline
\end{tabular}
}
\end{table}

==> two_tables.tex <==


\begin{table*}[ht]
\centering
\begin{minipage}{0.48\textwidth}
\centering
\caption{The ROUGE-L results with generated examples by Self-instruct method (ChatGPT as the backbone; \citep{wang2023selfinstruct}) 
in zero-shot and few-shot settings on held-out dataset. }
\label{table3}
\vspace{1mm}
\renewcommand{\arraystretch}{1.4}
\resizebox{\linewidth}{!}{
  \begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Model Size} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Testing Setting →\\ Training Setting ↓\end{tabular}} & \multirow{2}{*}{Zero-Shot}         & \multirow{2}{*}{Few-Shot} & \multirow{2}{*}{Avg ROUGE-L} \\
                            &                                                                                                   &                                    &                           &                             \\ \hline
\multirow{2}{*}{770M}       & SuperNI(Zero-Shot)                                                                                 & 32.66        & 37.50                    & 35.08                      \\ & SuperNI(Few-Shot)                                                                                 & 23.08        & 40.54                    & 31.81                      \\
                            & \mname                                                                                               & \textbf{32.62}                                   & \textbf{41.16}           & \textbf{36.89}         \\ \hline
\multirow{2}{*}{3B}         & SuperNI(Zero-Shot)                                                                                 & 37.63         & 41.53                    & 39.58                      \\ & SuperNI(Few-Shot)                                                                                 & 36.38         & 43.09                    & 39.73                      \\
                            & \mname                                                                                               & \textbf{37.95} & \textbf{44.23}            & \textbf{41.09}              \\ \bottomrule
\end{tabular}}
  \vspace{2mm}
\end{minipage}
\hspace*{1em}
\begin{minipage}{0.48\textwidth}
\centering
\caption{The ROUGE-L results for different stages in zero-shot and few-shot settings on held-out dataset. \textbf{Separated:} divide classification and answering into two independent stages. \textbf{Combined:} thinking first, answering later.}
\label{table4}
\renewcommand{\arraystretch}{1}
\resizebox{\linewidth}{!}{
  \begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Model size} & \multirow{2}{*}{Stage} & \multicolumn{1}{l}{\multirow{2}{*}{Zero-Shot}} & \multirow{2}{*}{Few-Shot} & \multirow{2}{*}{Avg ROUGE-L} \\
                            &                        & \multicolumn{1}{l}{}                           &                           &                             \\ \hline
\multirow{2}{*}{770M}       & Separated              & \textbf{40.69}                                & 29.11                    & 34.90                      \\
                            & Combined               & 33.58                                         & \textbf{46.66}           & \textbf{40.12}             \\ \hline
\multirow{2}{*}{3B}         & Separated              & 42.82                                         & 43.40                      & 43.11                      \\
                            & Combined               & \textbf{43.09}                                 & \textbf{52.11}           & \textbf{47.60}             \\ \bottomrule
\end{tabular}}
\end{minipage}
\end{table*}
